Growth of A Massive Black Hole Via Tidal Disruption Accretion

Stars that are tidally disrupted by the massive black hole (MBH) may contribute significantly to the growth of the MBH, especially in dense nuclear star clusters (NSCs). Yet, this tidal disruption accretion (TDA) of stars onto the MBH has largely been overlooked compared to the gas accretion (GA) channel in most numerical experiments until now. In this work, we implement a black hole growth channel via TDA in the high-resolution adaptive mesh refinement code Enzo to investigate its influence on a MBH seed's early evolution. We find that a MBH seed grows rapidly from $10^3\,\mathrm{M}_\odot$ to $\gtrsim 10^6\,\mathrm{M}_\odot$ in 200\,Myrs in some of the tested simulations. Compared to a MBH seed that grows only via GA, TDA can enhance the MBH's growth rate by up to more than an order of magnitude. However, as predicted, TDA mainly helps the early growth of the MBH (from $10^{3-4}\,\mathrm{M}_\odot$ to $\lesssim10^{5}\,\mathrm{M}_\odot$) while the later evolution is generally dominated by GA. We also observe that the star formation near the MBH is suppressed when TDA is most active, sometimes with a visible cavity in gas (of size $\sim$ a few pc) created in the vicinity of the MBH. It is because the MBH may grow expeditiously with both GA and TDA, and the massive MBH could consume its neighboring gas faster than being replenished by gas inflows. Our study demonstrates the need to consider different channels of black hole accretion that may provide clues for the existence of supermassive black holes at high redshifts.

==> sub.tex <==
\appendix

\section{A brief story toward a massive black hole seed in a dense star cluster}
The formation of an MBH seed in a dense star cluster has been widely discussed \citep{Fabian1975MNRAS.172P..15F, Sanders1970ApJ...162..791S, Begelman1978MNRAS.185..847B, Quinlan1987ApJ...321..199Q, Ebisuzaki2001ApJ...562L..19E,Zwart2004Natur.428..724P, Gurkan2004ApJ...604..632G, FreitagI2006MNRAS.368..121F,FreitageII2006MNRAS.368..141F, Miller2012ApJ...755...81M, Kremer2020ApJ...903...45K, Gonzalez2021ApJ...908L..29G}. A stellar system evolves toward an isothermal model, thus the core radius of the system begins to decrease while the density increases. This process is called a core-collapse. As a result of core collapse, the density of the core becomes extraordinarily dense. This can lead to the runaway merger and collision, and produce an MBH seed. The runaway seed formation scenarios can be distinguished into two (fast and slow) according to the speed of MBH seed formation.

However, there are some barriers such as the energy support from the binaries. Also, the resultant black hole from the merger of the binary may be ejected because of the gravitational kick \citep{Holley2008ApJ...686..829H}. \cite{Miller2002MNRAS.330..232C} showed that the core of the cluster with velocity dispersion $\sigma \gtrsim 40\,\mathrm{km}\,\mathrm{s}^{-1}$ can still collapse since the energy of the binary is not sufficient to prevent the collapse. They also pointed out that the clusters with velocity dispersion $\sigma \gtrsim 100\ \rm km \ \rm s^{-1}$ can keep the resultant black hole from being ejected by the GW kick. Star clusters with $40\,\mathrm{km/s} \lesssim \sigma \lesssim 100\,\mathrm{km/s}$ may still hold the merger product. Even for the case where no black hole remains, the runaway stellar merger can produce a black hole afterward. To summarize, a dense star cluster may form an MBH seed through several paths.

\subsection{Fast runaway formation}
% Fast runaway formation이 일어나기 위한 조건
The typical timescale of core collapse is roughly $t_\mathrm{cc} \simeq 15 t_\mathrm{rh}$. The stellar mass spectrum may lead to a faster core collapse. Core collapse continues until either the binary in the core or the merger product is massive enough to supply enough heat energy. \cite{Miller2002MNRAS.330..232C} argued that binary heating cannot prevent the core collapse of star clusters with a velocity dispersion $\sigma \gtrsim 40\,\mathrm{km}/\mathrm{s}$. Above this limit, the shrinking core forms a super-dense stellar environment. In this region, the frequent mergers and tidal disruption events may lead to an MBH seed. The resultant black hole from the merger of the binary may be ejected because of the gravitational kick \citep{Holley2008ApJ...686..829H}. Therefore, \cite{Miller2012ApJ...755...81M} also pointed that $\sigma \gtrsim 100\,\mathrm{km/s}$ is required to prevent the ejection. However, even though zero or one MBH remains after merger, a frequent star-star or star-BH interactions can still form an IMBH seed \citep{Zwart2002ApJ...576..899P, Gurkan2004ApJ...604..632G, FreitagI2006MNRAS.368..121F, FreitageII2006MNRAS.368..141F}.

The IMBH seed mass in a star cluster can be estimated with several approaches. \cite{Gurkan2004ApJ...604..632G} pointed out that a ever-collapsing core may contain a nonzero mass,
\begin{equation}
    M_\mathrm{cc} \simeq 0.001 - 0.002 M_\mathrm{tot}
\end{equation}
Where $M_\mathrm{tot}$ refers to the total mass of the star cluster. Assuming that the mass of the central black hole is enough to stop further core collapse and the black hole has negligible movements, \cite{Miller2012ApJ...755...81M} suggested two different lower bounds of the black hole mass
\begin{equation}
    M_\mathrm{BH} \gtrsim 500 \mathrm{M}_\odot \left(\sigma/40\,\mathrm{km} \mathrm{s}^{-1} \right)^{-4}
\label{eq: minimal threshold 1}
\end{equation}
and
\begin{equation}
   M_\mathrm{BH} \gtrsim 2 \times 10^3 \mathrm{M}_\odot \left(\sigma / 40\,\mathrm{km}\,\mathrm{s}^{-1}\right)^{8/3}.
\end{equation}
Given the scaling relation between the mass and the velocity dispersion of the star cluster, these criteria result in a similar mass of a typical NSC $10^6 \mathrm{M}_\odot \lesssim M_\mathrm{NSC} \lesssim 10^8 \mathrm{M}_\odot$.

% IMBH seed가 만들어진 후.
After an IMBH seed is formed, it prevents further collapse of the star cluster while it consumes nearby stars. Therefore, the stellar density nearby the seed evolves toward a steady-state \citep[e.g.][]{Bahcall1976ApJ...209..214B}. This behaviour is supported by the Monte Carlo simulations of \cite{Marchant1980ApJ...239..685M}. They showed that the appearance of black hole seed increases the core size while the mass of the MBH grows rapidly during the core re-expansion era.


\subsection{Slow runaway formation}
The slow runaway scenario is well explained by \cite{Stone2015ApJ...806L..28S}. When a star cluster failed to fully collapse, it can still have a dense core (but less dense and larger core compared to a fully collapsed case). Within this dense core, stellar mass black holes wander around the core and tidally captures nearby stars. As the black hole grows, its wander radius decreases and begins to dominate nearby stars. During this era, the star consumption rate of black hole scales as $\dot{M}_\mathrm{BH} \propto M_\mathrm{BH}^{4/3}$. This trend continues when $r_\mathrm{crit} < r_\mathrm{BH}$. After the fast/slow runaway seed formation, the black hole seed can grow by consuming both gas and star. Our goal is to trace the growth history of the IMBH seed after the runaway process.

\section{Brief Loss Cone Theory}
\label{sec: loss cone theory}

Suppose a star with a distance $r$ from an MBH. Its orbit would encounter the tidal radius if the angular momentum is small enough. Such orbit is said to lie within a loss cone \citep{Lightman1977ApJ...211..244L, Young1977ApJ...212..367Y}. In the loss cone theory the star lying within the loss cone is assumed to be removed.

The loss process is divided into two 

The rate, $\dot{N}_\mathrm{TD}$ can be obtained by adding the TDR of the empty loss cone $\dot{N}_\mathrm{empty}$ and the TDR of the full loss cone $\dot{N}_\mathrm{full}$ \citep{Syer1999MNRAS.306...35S}.
\begin{equation}
    \dot{N}_\mathrm{TD} = \dot{N}_\mathrm{full} + \dot{N}_\mathrm{empty}
\end{equation}
The full loss cone is the regime where the diffusion timescale $T_\mathrm{r}$ is short enough such that the loss cone is refilled within a short time. Conversely, the empty loss cone is the regime where the diffusion timescale is much longer than the dynamical timescale such that the loss cone is not refilled quickly. In most cases, it is known that the empty loss cone dominates the TDR. The radius where $\dot{N}_\mathrm{full}$ equals to $\dot{N}_\mathrm{empty}$ is the critical radius, $r_\mathrm{crit}$. If $r_\mathrm{crit} \gg r_\mathrm{BH}$, the TDR is approximately
\begin{equation}
    \dot{N}_\mathrm{TD} \approx \frac{N\left(r_\mathrm{BH}\right)}{t_\mathrm{R}\left(r_\mathrm{BH}\right)}.
\label{eq: TDR 1}
\end{equation}
On the other hand, if $r_\mathrm{crit} \ll r_\mathrm{BH}$, then the TDR is approximately
\begin{equation}
    \dot{N}_\mathrm{TD} \approx \frac{N\left(r_\mathrm{crit}\right)}{t_\mathrm{R}\left(r_\mathrm{crit}\right)}.
\label{eq: TDR 2}
\end{equation}
However, in the mass range of $M_\mathrm{BH}$ within our interest, $r_\mathrm{crit} \ll r_\mathrm{BH}$. Therefore, we only consider the rates according to Equation \ref{eq: TDR 2}.

If a star comes within a tidal radius
\begin{equation}
    r_\mathrm{t} = \left(\eta^2 \frac{M_\mathrm{BH}}{M_*}\right)^{1/3}r_*
\end{equation}
of the black hole, it is tidally disrupted. For the black holes with mass $\leq \mathrm{few} \times 10^7 \mathrm{M}_\odot$, the tidal radius is larger than the Schwarzschild radius. We define a 'loss cone' as the family of orbits with pericenters less than black hole tidal radius. Then the stars whose orbit lie within the loss cone are likely to be tidally disrupted. In a spherical star cluster we can say that the star will be consumed if
\begin{equation}
    J^2 \leq J^2_\mathrm{lc}\left(\epsilon\right)\equiv 2r^2_\mathrm{t}\left[\psi\left(2 r_\mathrm{t}\right) - \epsilon\right] \simeq 2GM_\mathrm{BH}r_\mathrm{t}
\end{equation}
\cite{Cohn1978ApJ...226.1087C} provides a formula to compute the stellar flux into the loss cone. The number of star income per unit time unit energy can be calculated by 
\begin{equation}
\mathcal{F}\left(\epsilon\right) d\epsilon = 4\pi^2 J_\mathrm{c}^2\left[\oint \frac{dr}{v_\mathrm{r}}\lim_{R\rightarrow 0} \frac{\left<\left(\Delta R\right)^2\right>}{2R}\right]\frac{f}{\ln{R_0}^{-1}}d\epsilon
\end{equation}
where $R \equiv J^2/J^2_\mathrm{c}\left(\epsilon\right)$ is the diffusion coefficient and $J_\mathrm{c}\left(\epsilon\right)$ is the angular momentum of a circular orbit of energy $\epsilon$. $R_0$ is the value of R at which $f$ becomes 0 due to the tidal removal of stars. According to \cite{Cohn1978ApJ...226.1087C}, the approximate value of $R_0\left(\epsilon\right)$ can by


Then the rate of tidal disruption is obtained by integration;
\begin{equation}
    \dot{N} = \int \mathcal{F}\left(\epsilon\right) d\epsilon.
\end{equation}

